Multi-scale speaker embedding-based graph attention networks for speaker diarisation

The objective of this work is effective speaker diarisation using multi-scale speaker embeddings. Typically, there is a trade-off between the ability to recognise short speaker segments and the discriminative power of the embedding, according to the segment length used for embedding extraction. To this end, recent works have proposed the use of multi-scale embeddings where segments with varying lengths are used. However, the scores are combined using a weighted summation scheme where the weights are fixed after the training phase, whereas the importance of segment lengths can differ with in a single session. To address this issue, we present three key contributions in this paper: (1) we propose graph attention networks for multi-scale speaker diarisation; (2) we design scale indicators to utilise scale information of each embedding; (3) we adapt the attention-based aggregation to utilise a pre-computed affinity matrix from multi-scale embeddings. We demonstrate the effectiveness of our method in various datasets where the speaker confusion which constitutes the primary metric drops over 10% in average relative compared to the baseline.

==> tables/all.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & MS & SC\\ 
	 \Xhline{1pt}
	 \multicolumn{5} {c} {\bf{DIHARD I} }\\
     \hline
    \Xhline{1pt}
	 Baseline (500ms) & 31.68 & 0.0 & 8.71 & 22.97 \\
	 Baseline (1000ms) & 22.29 & 0.0 & 8.71 & 13.58 \\
	 Baseline (1500ms) & 20.54 & 0.0 & 8.71 & 11.83 \\
	 \hline
	 AM-Fusion & 23.44 & 0.0 & 8.71 & 14.72 \\
	 GATs & {\bf{19.00}} & 0.0 & 8.71 & 10.29 \\
	 \hline
	 Track winner \cite{sell2018diarization} & 23.73 & - & - & - \\
    \Xhline{1pt}
    \multicolumn{5} {c} {\bf{DIHARD II} }\\
     \Xhline{1pt}
     Baseline (500ms) & 35.28 & 0.0 & 9.69 & 25.59 \\
	 Baseline (1000ms) & 22.77 & 0.0 & 9.69 & 13.08 \\
	 Baseline (1500ms) & 21.47 & 0.0 & 9.69 & 11.78 \\
	 \hline
	 AM-Fusion & 23.10 & 0.0 & 9.69 & 13.41 \\
	 GATs & 19.8 & 0.0 & 9.69 & 10.12 \\
	 \hline
	 Track winner \cite{landini2019but} & {\bf{18.42}} & - & - & - \\
    \Xhline{1pt}
    \multicolumn{5} {c} {\bf{DIHARD III} }\\
    \Xhline{1pt}
     Baseline (500ms) & 25.01 & 0.0 & 9.52 & 15.49 \\
	 Baseline (1000ms) & 17.50 & 0.0 & 9.52 & 7.98 \\
	 Baseline (1500ms) & {\bf{17.04}} & 0.0 & 9.52 & 7.52 \\
	 \hline
	 AM-Fusion & 18.25 & 0.0 & 9.52 & 8.73 \\
	 GATs & 17.35 & 0.0 & 9.52 & 7.83 \\
    \Xhline{1pt}
    \multicolumn{5} {c} {\bf{VoxConverse} }\\
    \Xhline{1pt}
    Baseline (500ms) & 28.76 & 1.38 & 3.29 & 24.08 \\
	 Baseline (1000ms) & 21.64 & 1.38 & 3.29 & 16.96 \\
	 Baseline (1500ms) & 14.88 & 1.38 & 3.29 & 10.21 \\
	 \hline
	 AM-Fusion & 18.95 & 1.38 & 3.29 & 14.27 \\
	 GATs & {\bf{12.78}} & 1.38 & 3.29 & 8.1 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	  Results on the DIHARD I, II, III and VoxConverse test sets.  (FA: false alarm, MS: miss, SC: speaker confusion, \textbf{lower is better for all four metrics}).  
	}
 	%\vspace{-10pt}
	\label{tab:results}
\end{table}

==> tables/dihard1.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & Miss & Conf\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 31.40 & 0.0 & 8.71 & 22.69 \\
	 Baseline (1000ms) & 25.46 & 0.0 & 8.71 & 16.75 \\
	 Baseline (1500ms) & 24.60 & 0.0 & 8.71 & 15.88 \\
	 \hline
	 AM-Fusion & 25.89 & 0.0 & 8.71 & 17.18 \\
	 GNN & 23.26 & 0.0 & 8.71 & 14.55 \\
	 GNN + AA & 19.00 & 0.0 & 8.71 & 10.29 \\
	 \hline
	 Track winner & 23.73 & - & - & - \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	  Effectiveness of the multiscale GATs when applied to the speaker diarisation pipeline using the DIHARD I test set track 1 configuration (FA: false alarm, Conf: confusion, \textbf{lower is better for all four metrics}).  
	}
 	%\vspace{-10pt}
	\label{tab:dihard1}
\end{table}

==> tables/dihard1_aa.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & MS & SC\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 31.68 & 0.0 & 8.71 & 22.97 \\
	 Baseline (1000ms) & 22.29 & 0.0 & 8.71 & 13.58 \\
	 Baseline (1500ms) & 20.54 & 0.0 & 8.71 & 11.83 \\
	 \hline
	 AM-Fusion & 23.44 & 0.0 & 8.71 & 14.72 \\
	 GATs & 19.00 & 0.0 & 8.71 & 10.29 \\
	 \hline
	 Track winner & 23.73 & - & - & - \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	  Effectiveness of the multiscale GATs when applied to the speaker diarisation pipeline using the DIHARD I test set track 1 configuration (FA: false alarm, MS: miss, SC: speaker confusion, \textbf{lower is better for all four metrics}).  
	}
 	%\vspace{-10pt}
	\label{tab:dihard1_aa}
\end{table}

==> tables/dihard2.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & Miss & Conf\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 35.61 & 0.0 & 9.69 & 25.93 \\
	 Baseline (1000ms) & 27.60 & 0.0 & 9.69 & 17.91 \\
	 Baseline (1500ms) & 27.87 & 0.0 & 9.69 & 18.18 \\
	 \hline
	 AM-Fusion & 28.13 & 0.0 & 9.69 & 18.44 \\
	 GNN & 22.85 & 0.0 & 9.69 & 13.16 \\
	 GNN + AA & 19.8 & 0.0 & 8.71 & 10.12 \\
	 \hline
	 Track winner & 18.42 & - & - & - \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	 the DIHARD II test set track 1 configuration.  
	}
 	%\vspace{-10pt}
	\label{tab:dihard2}
\end{table}

==> tables/dihard2_aa.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & MS & SC\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 35.28 & 0.0 & 9.69 & 25.59 \\
	 Baseline (1000ms) & 22.77 & 0.0 & 9.69 & 13.08 \\
	 Baseline (1500ms) & 21.47 & 0.0 & 9.69 & 11.78 \\
	 \hline
	 AM-Fusion & 23.10 & 0.0 & 9.69 & 13.41 \\
	 GATs & 19.8 & 0.0 & 9.69 & 10.12 \\
	 \hline
	 Track winner & 18.42 & - & - & - \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	 the DIHARD II test set track 1 configuration.  
	}
 	%\vspace{-10pt}
	\label{tab:dihard2_aa}
\end{table}

==> tables/dihard3.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & Miss & Conf\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 25.15 & 0.0 & 9.52 & 15.62 \\
	 Baseline (1000ms) & 20.08 & 0.0 & 9.52 & 10.56 \\
	 Baseline (1500ms) & 19.93 & 0.0 & 9.52 & 10.40 \\
	 \hline
	 AM-Fusion & 20.48 & 0.0 & 9.52 & 10.96 \\
	 GNN & 18.32 & 0.0 & 9.52 & 8.79 \\
	 GNN + AA & 17.35 & 0.0 & 9.52 & 7.83 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	  the DIHARD III test set track 1 configuration.  
	}
 	%\vspace{-10pt}
	\label{tab:dihard3}
\end{table}

==> tables/dihard3_aa.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & MS & SC\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 25.01 & 0.0 & 9.52 & 15.49 \\
	 Baseline (1000ms) & 17.50 & 0.0 & 9.52 & 7.98 \\
	 Baseline (1500ms) & 17.04 & 0.0 & 9.52 & 7.52 \\
	 \hline
	 AM-Fusion & 18.25 & 0.0 & 9.52 & 8.73 \\
	 GATs & 17.35 & 0.0 & 9.52 & 7.83 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
	  the DIHARD III test set track 1 configuration.  
	}
 	%\vspace{-10pt}
	\label{tab:dihard3_aa}
\end{table}

==> tables/gnn_ablation.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYYY}
    \Xhline{1pt}
	Configuration & DER & FA & MS & SC \\ 
    \Xhline{1pt}
     \multicolumn{5} {c} {\bf{DIHARD I} }\\
     \hline
     GATs & 30.53 & 0.0 & 8.71 & 21.81 \\
     GATs + Pos & 23.26 & 0.0 & 8.71 & 14.55 \\
	 GATs + Pos + AA & 19.00 & 0.0 & 8.71 & 10.29 \\
	 \hline
	 \multicolumn{5} {c} {\bf{DIHARD II} }\\
     \hline
     GATs & 28.98 & 0.0 & 9.69 & 19.29 \\
	 GATs + Pos & 22.85 & 0.0 & 9.69 & 13.16 \\
	 GATs + Pos + AA & 19.8 & 0.0 & 8.71 & 10.12 \\
	 \hline
	 \multicolumn{5} {c} {\bf{DIHARD III} }\\
     \hline
     GATs & 22.83 & 0.0 & 9.52 & 13.31 \\
	 GATs + Pos & 18.32 & 0.0 & 9.52 & 8.79 \\
	 GATs + Pos + AA & 17.35 & 0.0 & 9.52 & 7.83 \\
	 \hline
	 \multicolumn{5} {c} {\bf{VoxConverse} }\\
     \hline
     GATs & 32.61 & 1.38 & 3.29 & 27.93 \\
	 GATs + Pos & 18.61 & 1.38 & 3.29 & 13.94 \\
	 GATs + Pos + AA & 12.78 & 1.38 & 3.29 & 8.1 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{Ablation study.  
	}
 	%\vspace{-10pt}
	\label{tab:gnn_ablation}
\end{table}

==> tables/voxconverse.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & Miss & Conf\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 28.94 & 1.38 & 3.29 & 24.26 \\
	 Baseline (1000ms) & 23.99 & 1.38 & 3.29 & 19.31 \\
	 Baseline (1500ms) & 24.80 & 1.38 & 3.29 & 20.12 \\
	 \hline
	 AM-Fusion & 22.98 & 1.38 & 3.29 & 18.30 \\
	 GNN & 18.61 & 1.38 & 3.29 & 13.94 \\
	 GNN + AA & 12.78 & 1.38 & 3.29 & 8.1 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
VoxConverse test set.  
	}
 	%\vspace{-10pt}
	\label{tab:voxconverse}
\end{table}

==> tables/voxconverse_aa.tex <==
\begin{table}[!t]
	\centering
	\small
	\begin{tabularx}{\columnwidth}{lYYYY}
    \Xhline{1pt}
	 Configuration & DER & FA & MS & SC\\ 
    \Xhline{1pt}
	 Baseline (500ms) & 28.76 & 1.38 & 3.29 & 24.08 \\
	 Baseline (1000ms) & 21.64 & 1.38 & 3.29 & 16.96 \\
	 Baseline (1500ms) & 14.88 & 1.38 & 3.29 & 10.21 \\
	 \hline
	 AM-Fusion & 18.95 & 1.38 & 3.29 & 14.27 \\
	 GATs & 12.78 & 1.38 & 3.29 & 8.1 \\
    \Xhline{1pt}
	\end{tabularx}
	\caption{
VoxConverse test set.  
	}
 	%\vspace{-10pt}
	\label{tab:voxconverse_aa}
\end{table}
